Zero-Shot Sign Language Recognition: Can Textual Data Uncover Sign Languages?

We introduce the problem of zero-shot sign language recognition (ZSSLR), where the goal is to leverage models learned over the seen sign class examples to recognize the instances of unseen signs. To this end, we propose to utilize the readily available descriptions in sign language dictionaries as an intermediate-level semantic representation for knowledge transfer. We introduce a new benchmark dataset called ASL-Text that consists of 250 sign language classes and their accompanying textual descriptions. Compared to the ZSL datasets in other domains (such as object recognition), our dataset consists of limited number of training examples for a large number of classes, which imposes a significant challenge. We propose a framework that operates over the body and hand regions by means of 3D-CNNs, and models longer temporal relationships via bidirectional LSTMs. By leveraging the descriptive text embeddings along with these spatio-temporal representations within a zero-shot learning framework, we show that textual data can indeed be useful in uncovering sign languages. We anticipate that the introduced approach and the accompanying dataset will provide a basis for further exploration of this new zero-shot learning problem.

==> Makefile <==
######################################################################
# Makefile for compiling tex files and setting up sharing permissions.
# Customized by Gokberk Cinbis based on many existing Makefile examples available online.
# Last update: May 2017
# 
# Requires a second, project-specific file named "Makefile.mk" that contains the following definitions:
# TEXFILE=<tex filename>    --> Nmae of the main tex file
# TITLE=<project title>     --> Name of the project
# PDFDIR=<output directory> --> OPTIONAL. The pdf output directory. 
#				(Use "." to compile in the source directory)
# 
# -- Example Makefile.mk --
# TEXFILE=paper.tex	
# TITLE=author17journal	
#
# Also supports the following environement variables:
# PDFDIR: The default value for the PDFDIR
# 
# If PDFDIR is not defined in Makefile.mk OR as an environment variable, "." is used.
# 

######################################################################

PDFDIRDEFAULT="$(PDFDIR)" # From the environement variable

include Makefile.mk # may or maynot overwrite PDFDIR

# if PDFDIR is undefined OR '', then use the current directory.
PDFDIR?=.
ifeq "$(PDFDIR)" ""
    PDFDIR=.
endif
ifneq "$(PDFDIR)" "."
    PDFDIR:=$(PDFDIR)/$(TITLE)
endif
FINALPDFFILE="$(PDFDIR)/$(TEXFILE:.tex=_stable.pdf)"

CMDPDFMAIN=pdflatex -output-directory $(PDFDIR) $(TEXFILE)
CMDPDF=$(CMDPDFMAIN) -file-line-error -interaction=nonstopmode | grep -i -e warn -e error -e pages -B4 -A4 -e '^l.' -e '^?' # hangs in cygwin in interactive mode
#CMDPDF=$(CMDPDFMAIN) -interaction=nonstopmode

#all:	export pdf bib share echo 
all:	pdfnonstop bib echo 
	@( \
	set -e; \
	if grep -q Error $(PDFDIR)/$(TEXFILE:.tex=.log); \
	then \
	    echo "SKIPPED COPYING THE PDF FILE TO AVOID PDF-READER CRASH, AS LOG CONTAINS ERROR"; \
	else \
	    mv -f $(PDFDIR)/$(TEXFILE:.tex=.pdf) $(FINALPDFFILE); \
	fi \
	)
	@#cp -f $(PDFDIR)/$(TEXFILE:.tex=.pdf) .

warn:	pdfnonstopwarnonly 

error:	pdferror bib echo

sup:	
	pdflatex supmat.tex
	bibtex supmat

echo:
	@echo "Tex file:$(TEXFILE)"
	@echo "Output files are under:$(PDFDIR)"
	@echo "Final pdf file:$(FINALPDFFILE)"

view:	all
	$(PDFVIEW) $(FINALPDFFILE) &

showlog: 	
	vi $(PDFDIR)/$(TEXFILE:.tex=.log)

open:	
	$(OPEN) $(PDFDIR) &

ps:	$(TEXFILE:.tex=.ps)
dvi:	$(TEXFILE:.tex=.dvi)
bib:	pdfnonstop bibrule

bibrule:	$(TEXFILE)
	@( \
	echo ================= bib ======================; \
	export openout_any=a; \
	bibtex "$(PDFDIR)/$(<:.tex=)"; \
	)

%.dvi: %.tex checkdep
	@( \
	echo ================= latex ======================; \
	latex $<; \
	while grep -q "Rerun to get cross-references right." $(<:.tex=.log); \
	do \
		echo ================= latex loop ======================; \
		latex $<; \
	done \
	)

%.ps: %.dvi
	@dvips -q -t a4 $< -o $(<:.dvi=.ps)

latex:	$(TEXFILE:.tex=.ps)
	@ps2pdf -dPDFSETTINGS=/prepress $<

# Note: $< is the first dependency.
#
# pdflatex -interaction=batchmode -halt-on-error -file-line-error $(TEXFILE); 
# use "X" to quit.
# 
# output-directory should be before the filename.
# pdflatex -file-line-error -output-directory $(PDFDIR) $(<); 
#
# Don't stop on errors
pdfnonstop:$(TEXFILE) checkdep 
	@( \
	echo ================= pdflatex ======================; \
	mkdir -p $(PDFDIR); \
	$(CMDPDF); \
	while grep -q "Rerun to get" $(PDFDIR)/$(<:.tex=.log); \
	do \
		echo ================= pdflatex loop ======================; \
		$(CMDPDF); \
	done \
	)

# Don't stop on errors, show warnings only
pdfnonstopwarnonly:$(TEXFILE) checkdep 
	@( \
	echo ================= pdflatex ======================; \
	mkdir -p $(PDFDIR); \
	$(CMDPDF) | grep Warn; \
	while grep -q "Rerun to get" $(PDFDIR)/$(<:.tex=.log); \
	do \
		echo ================= pdflatex loop ======================; \
		$(CMDPDF) | grep Warn; \
	done \
	)


# Stop on errors
pdferror: 	$(TEXFILE) checkdep 
	@( \
	echo ================= pdflatex ======================; \
	mkdir -p $(PDFDIR); \
	$(CMDPDFMAIN); \
	while grep -q "Rerun to get" $(PDFDIR)/$(<:.tex=.log); \
	do \
		echo ================= pdflatex loop ======================; \
		$(CMDPDFMAIN); \
	done \
	)

compress:
	@(cd $(PDFDIR) && ls -alh $(TEXFILE:.tex=.pdf) && pdf2ps $(TEXFILE:.tex=.pdf) && ps2pdf $(TEXFILE:.tex=.ps) && ls -alh $(TEXFILE:.tex=.pdf) && rm -f ps2pdf $(TEXFILE:.tex=.ps))

share:	
	@find . -user ${USER} -type d -execdir chmod 770 "{}" \;
	@find . -user ${USER} -type f -execdir chmod 660 "{}" \;

# check whether bibtex changed the bibliography file
checkdep: $(TEXFILE:.tex:.aux) 

export:	
	@bash export.sh

watch:
	watch -n 600 git pull

clean:
	@rm -f {./,$(PDFDIR)/}$(TEXFILE:.tex=.){aux,log,out,dvi,pdf,bbl,blg,ps,brf,lof,lot,nlo,maf,toc} 
	@rm -f {./,$(PDFDIR)/}$(TEXFILE:.tex=.){mlc,mlt,mtc,mlf}*



==> macros.tex <==
% based on Jakob Verbeek's macros.tex

\usepackage{color}
\usepackage[normalem]{ulem}

\def\etal{et al.\ }
\def\Eq#1{Eq.~(\ref{eq:#1})}

\usepackage{amsmath,amssymb,amsbsy,xspace}
\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}

\def\eg{\emph{e.g}\onedot} \def\Eg{\emph{E.g}\onedot}
\def\ie{\emph{i.e}\onedot} \def\Ie{\emph{I.e}\onedot}
\def\cf{\emph{c.f}\onedot} \def\Cf{\emph{C.f}\onedot}
\def\etc{\emph{etc}\onedot} \def\vs{\emph{vs}\onedot} 
\def\wrt{w.r.t\onedot} \def\dof{d.o.f\onedot}
\def\etal{\emph{et al}\onedot}

\def\Eqs#1{Eqs.~(\ref{eq:#1})}
\def\Eq#1{Eq.~(\ref{eq:#1})}
\def\eq#1{(\ref{eq:#1})}
\def\be{\begin{equation}}
\def\ee{\end{equation}}
\def\bea{\begin{eqnarray}}
\def\eea{\end{eqnarray}}
\def\fig#1{Figure~\ref{fig:#1}}
\def\tab#1{Table~\ref{tab:#1}}
\def\sect#1{Section~\ref{sec:#1}}
\def\chap#1{Chapter~\ref{chap:#1}}
\def\app#1{Appendix~\ref{app:#1}}
\def\algo#1{Algorithm~\ref{algo:#1}}

\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
%\newcommand{\argmin}{\operatornamewithlimits{argmin}}
%\newcommand{\argmax}{\operatornamewithlimits{argmax}}

\makeatother

\newcommand{\myparagraphwospace}[1]{\noindent{\bf #1}} 
\newcommand{\myparagraphwithspace}[1]{\vspace{6pt}\noindent{\bf #1}} 


